Young wall realizations of level 1 irreducible highest weight and Fock space crystals of quantum affine algebras in type E

We construct Young wall models for the crystal bases of level $1$ irreducible highest weight representations and Fock space representations of quantum affine algebras in types $E_{6}^{(1)}$, $E_{7}^{(1)}$ and $E_{8}^{(1)}$. In each case, Young walls consist of coloured blocks stacked inside the relevant Young wall pattern which satisfy a certain combinatorial condition. Moreover the crystal structure is described entirely in terms of adding and removing blocks.

==> wall_1.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=none] (0,0) rectangle ++(2,2);
    \node[color=black] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=none] (0,4) rectangle ++(2,4);
    \node[color=black] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=none] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=black] at (1,9) {\footnotesize $4$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=none] (-4,0) rectangle ++(2,2);
    \node[color=black] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};

==> wall_10.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=col0] (0,0) rectangle ++(2,2);
    \node[color=white] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=col2] (0,4) rectangle ++(2,4);
    \node[color=white] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=col4] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=white] at (1,9) {\footnotesize $4$};

    \draw[fill=col3] (0,12) rectangle ++(2,4);
    \node[color=white] at (1,14) {\footnotesize $3$};
    \draw[fill=col5] (2,12) rectangle ++(2,4);
    \node[color=white] at (3,14) {\footnotesize $5$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);
    \draw[line width = 1.5] (0,12) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=col6] (-4,0) rectangle ++(2,2);
    \node[color=white] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};

==> wall_11.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=col0] (0,0) rectangle ++(2,2);
    \node[color=white] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=col2] (0,4) rectangle ++(2,4);
    \node[color=white] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=col4] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=white] at (1,9) {\footnotesize $4$};

    \draw[fill=col3] (0,12) rectangle ++(2,4);
    \node[color=white] at (1,14) {\footnotesize $3$};
    \draw[fill=col5] (2,12) rectangle ++(2,4);
    \node[color=white] at (3,14) {\footnotesize $5$};

    \draw[fill=none] (0,16) rectangle ++(2,2);
    \node[color=black] at (1,17) {\footnotesize $1$};
    \draw[fill=col4] (0,18) |- (4,20) |- (2,16) |- cycle;
    \node[color=white] at (3,19) {\footnotesize $4$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);
    \draw[line width = 1.5] (0,12) rectangle ++(4,4);
    \draw[line width = 1.5] (0,16) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=none] (-4,0) rectangle ++(2,2);
    \node[color=black] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};

==> wall_12.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=col0] (0,0) rectangle ++(2,2);
    \node[color=white] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=col2] (0,4) rectangle ++(2,4);
    \node[color=white] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=col4] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=white] at (1,9) {\footnotesize $4$};

    \draw[fill=col3] (0,12) rectangle ++(2,4);
    \node[color=white] at (1,14) {\footnotesize $3$};
    \draw[fill=col5] (2,12) rectangle ++(2,4);
    \node[color=white] at (3,14) {\footnotesize $5$};

    \draw[fill=col1] (0,16) rectangle ++(2,2);
    \node[color=white] at (1,17) {\footnotesize $1$};
    \draw[fill=none] (0,18) |- (4,20) |- (2,16) |- cycle;
    \node[color=black] at (3,19) {\footnotesize $4$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);
    \draw[line width = 1.5] (0,12) rectangle ++(4,4);
    \draw[line width = 1.5] (0,16) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=none] (-4,0) rectangle ++(2,2);
    \node[color=black] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};

==> wall_2.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=col0] (0,0) rectangle ++(2,2);
    \node[color=white] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=none] (0,4) rectangle ++(2,4);
    \node[color=black] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=none] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=black] at (1,9) {\footnotesize $4$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=none] (-4,0) rectangle ++(2,2);
    \node[color=black] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};

==> wall_3.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=col0] (0,0) rectangle ++(2,2);
    \node[color=white] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=col2] (0,4) rectangle ++(2,4);
    \node[color=white] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=none] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=black] at (1,9) {\footnotesize $4$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=none] (-4,0) rectangle ++(2,2);
    \node[color=black] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};

==> wall_4.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=col0] (0,0) rectangle ++(2,2);
    \node[color=white] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=col2] (0,4) rectangle ++(2,4);
    \node[color=white] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=col4] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=white] at (1,9) {\footnotesize $4$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=none] (-4,0) rectangle ++(2,2);
    \node[color=black] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};

==> wall_5.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=col0] (0,0) rectangle ++(2,2);
    \node[color=white] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=col2] (0,4) rectangle ++(2,4);
    \node[color=white] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=col4] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=white] at (1,9) {\footnotesize $4$};

    \draw[fill=none] (0,12) rectangle ++(2,4);
    \node[color=black] at (1,14) {\footnotesize $3$};
    \draw[fill=col5] (2,12) rectangle ++(2,4);
    \node[color=white] at (3,14) {\footnotesize $5$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);
    \draw[line width = 1.5] (0,12) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=none] (-4,0) rectangle ++(2,2);
    \node[color=black] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};

==> wall_6.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=col0] (0,0) rectangle ++(2,2);
    \node[color=white] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=col2] (0,4) rectangle ++(2,4);
    \node[color=white] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=col4] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=white] at (1,9) {\footnotesize $4$};

    \draw[fill=col3] (0,12) rectangle ++(2,4);
    \node[color=white] at (1,14) {\footnotesize $3$};
    \draw[fill=none] (2,12) rectangle ++(2,4);
    \node[color=black] at (3,14) {\footnotesize $5$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);
    \draw[line width = 1.5] (0,12) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=none] (-4,0) rectangle ++(2,2);
    \node[color=black] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};

==> wall_7.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=col0] (0,0) rectangle ++(2,2);
    \node[color=white] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=col2] (0,4) rectangle ++(2,4);
    \node[color=white] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=col4] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=white] at (1,9) {\footnotesize $4$};

    \draw[fill=none] (0,12) rectangle ++(2,4);
    \node[color=black] at (1,14) {\footnotesize $3$};
    \draw[fill=col5] (2,12) rectangle ++(2,4);
    \node[color=white] at (3,14) {\footnotesize $5$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);
    \draw[line width = 1.5] (0,12) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=col6] (-4,0) rectangle ++(2,2);
    \node[color=white] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};

==> wall_8.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=col0] (0,0) rectangle ++(2,2);
    \node[color=white] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=col2] (0,4) rectangle ++(2,4);
    \node[color=white] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=col4] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=white] at (1,9) {\footnotesize $4$};

    \draw[fill=col3] (0,12) rectangle ++(2,4);
    \node[color=white] at (1,14) {\footnotesize $3$};
    \draw[fill=col5] (2,12) rectangle ++(2,4);
    \node[color=white] at (3,14) {\footnotesize $5$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);
    \draw[line width = 1.5] (0,12) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=none] (-4,0) rectangle ++(2,2);
    \node[color=black] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};

==> wall_9.tex <==
    \node at (2,-2) {\Large $\vdots$};

    \draw[fill=col0] (0,0) rectangle ++(2,2);
    \node[color=white] at (1,1) {\footnotesize $0$};
    \draw[fill=col4] (0,2) |- (4,4) |- (2,0) |- cycle;
    \node[color=white] at (3,3) {\footnotesize $4$};

    \draw[fill=col2] (0,4) rectangle ++(2,4);
    \node[color=white] at (1,6) {\footnotesize $2$};
    \draw[fill=col5] (2,4) rectangle ++(2,4);
    \node[color=white] at (3,6) {\footnotesize $5$};

    \draw[fill=col6] (2,10) rectangle ++(2,2);
    \node[color=white] at (3,11) {\footnotesize $6$};
    \draw[fill=col4] (0,8) |- (2,12) |- (4,10) |- cycle;
    \node[color=white] at (1,9) {\footnotesize $4$};

    \draw[fill=col3] (0,12) rectangle ++(2,4);
    \node[color=white] at (1,14) {\footnotesize $3$};
    \draw[fill=none] (2,12) rectangle ++(2,4);
    \node[color=black] at (3,14) {\footnotesize $5$};

    \draw[fill=col1] (0,16) rectangle ++(2,2);
    \node[color=white] at (1,17) {\footnotesize $1$};
    \draw[fill=none] (0,18) |- (4,20) |- (2,16) |- cycle;
    \node[color=black] at (3,19) {\footnotesize $4$};

    \draw[line width = 1.5] (0,0) rectangle ++(4,4);
    \draw[line width = 1.5] (0,4) rectangle ++(4,4);
    \draw[line width = 1.5] (0,8) rectangle ++(4,4);
    \draw[line width = 1.5] (0,12) rectangle ++(4,4);
    \draw[line width = 1.5] (0,16) rectangle ++(4,4);

    \node at (-2,-2) {\Large $\vdots$};

    \draw[fill=none] (-4,0) rectangle ++(2,2);
    \node[color=black] at (-3,1) {\footnotesize $6$};
    \draw[fill=col4] (-4,2) |- (0,4) |- (-2,0) |- cycle;
    \node[color=white] at (-1,3) {\footnotesize $4$};

    \draw[fill=none] (-4,4) rectangle ++(2,4);
    \node[color=black] at (-3,6) {\footnotesize $5$};
    \draw[fill=col3] (-2,4) rectangle ++(2,4);
    \node[color=white] at (-1,6) {\footnotesize $3$};

    \draw[fill=col1] (-2,10) rectangle ++(2,2);
    \node[color=white] at (-1,11) {\footnotesize $1$};
    \draw[fill=none] (-4,8) |- (-2,12) |- (0,10) |- cycle;
    \node[color=black] at (-3,9) {\footnotesize $4$};

    \draw[line width = 1.5] (-4,0) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,4) rectangle ++(4,4);
    \draw[line width = 1.5] (-4,8) rectangle ++(4,4);

    \draw[line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-4cm, line width = 1.5] (4,-2) -- (4,0);
    \draw[xshift=-8cm, line width = 1.5] (4,-2) -- (4,0);

    \draw[line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=4cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=8cm, line width = 1.5] (4,0) -- (-6,0);
    \draw[yshift=12cm, line width = 1.5] (4,0) -- (-6,0);

    \node at (-6,2) {\large $\dots$};
    \node at (-6,6) {\large $\dots$};
    \node at (-6,10) {\large $\dots$};
